MistralBSM: Leveraging Mistral-7B for Vehicular Networks Misbehavior Detection

Malicious attacks on vehicular networks pose a serious threat to road safety as well as communication reliability. A major source of these threats stems from misbehaving vehicles within the network. To address this challenge, we propose a Large Language Model (LLM)-empowered Misbehavior Detection System (MDS) within an edge-cloud detection framework. Specifically, we fine-tune Mistral-7B, a compact and high-performing LLM, to detect misbehavior based on Basic Safety Messages (BSM) sequences as the edge component for real-time detection, while a larger LLM deployed in the cloud validates and reinforces the edge model's detection through a more comprehensive analysis. By updating only 0.012% of the model parameters, our model, which we named MistralBSM, achieves 98% accuracy in binary classification and 96% in multiclass classification on a selected set of attacks from VeReMi dataset, outperforming LLAMA2-7B and RoBERTa. Our results validate the potential of LLMs in MDS, showing a significant promise in strengthening vehicular network security to better ensure the safety of road users.

==> algo.tex <==
% \begin{algorithm}[!t]
% \caption{Federated YOLOv7}
% \label{alg:alg1}
%   \begin{algorithmic}[0]
%     \vspace{0.1cm}
%     \STATE \textbf{Input:} Communication rounds \(R\), local epochs \(E\), local mini-batch size \(B\), server learning rate \(\eta\), server momentum factor \(\beta \in [0, 1)\), YOLOv7 set of hyperparameters \(\mathcal{H}\).
%     \vspace{0.1cm}
%     \STATE \textbf{Output:} Best re-parameterized joint model \(w_{\text{r}}^{*}\).
%     \\\hrulefill
%     \vspace{0.1cm}
%     \STATE \textbf{Server \(\mathcal{S}\) executes:}
%     \begin{ALC@g}
%     \STATE Gather public key \(pk_{i}\) from each client \(\mathcal{C}_i\)
%     \STATE Initialize model \(w^{0}\) from pretrained weights
%     \STATE Initialize server-side momentum \(v^{0}=0\)
%     \FOR{\(t = 0, ..., R-1\)}
%         \STATE Initialize symmetric key \(sk^{t}\)
%         \STATE \(\{w^{t}\}\leftarrow\) Encrypt \(w^{t}\) with \(sk^{t}\)
%         \STATE \(\{sk^{t}\}_{i:1:m}\leftarrow\) Encrypt \(sk^{t}\) for each \(pk_{i}\)
%         \FOR{each client \(\mathcal{C}_i\) \textbf{in parallel}} 
%             \STATE\(\{\Delta_{i}^{t}\}\), \(n_{i} = \) \textbf{ClientUpdate}(\(\{w^{t}\}, \{sk^{t}\}_{i}, t\))
%         \ENDFOR
%         \STATE \(n = \sum_{i=1}^{m} n_{i}\)
%         \STATE \(\Delta_{i:1:m}^{t} \leftarrow\) Decrypt each \(\{\Delta_{i}^{t}\}\) with \(sk^{t}\)
%         \STATE \(\Delta^{t} = \sum_{i=1}^{m} \frac{n_{i}}{n}\Delta_{i}^{t}\)
%         \STATE \(v^{t+1} = \beta v^{t} + \Delta^{t}\)
%         \STATE \(w^{t+1} = w^{t} - \eta v^{t+1}\)
%         \STATE \(w_{\text{r}}^{t+1} = \texttt{reparameterize}(w^{t+1})\)
%         \STATE \(\text{Evaluation metrics} = \texttt{test}(w_{\text{r}}^{t+1}, \mathcal{D}_{\mathcal{S}}, \mathcal{H})\)
%     \ENDFOR
%     \STATE \textbf{return} \(w_{\text{r}}^{*}\) based on mAP
%     \end{ALC@g}
%     \vspace{0.1cm}
%     \STATE \textbf{ClientUpdate(\(\{w^{t}\}, \{sk^{t}\}_{i}, t\)):} \hspace{0.2cm} // \emph{run on client \(\mathcal{C}_i\)} 
%     \begin{ALC@g}
%         \STATE \(sk^{t} \leftarrow\) Decrypt \(\{sk^{t}\}_{i}\) with private key
%         \STATE \(w^{t} \leftarrow\) Decrypt \(\{w^{t}\}\) with \(sk^{t}\)
%         \STATE \(w_{i}^{t} = \texttt{train}(w^{t}, \mathcal{D}_{i}, E, B, \mathcal{H}, t)\)
%         \STATE \(\Delta_{i}^{t} = w^{t} - w_{i}^{t}\)
%         \STATE \(\{\Delta_{i}^{t}\} \leftarrow\) Encrypt \(\Delta_{i}^{t}\) with \(sk^{t}\)
%         \STATE \textbf{return} \(\{\Delta_{i}^{t}\}\), \(|\mathcal{D}_{i}|\) to server
%     \end{ALC@g}
%   \end{algorithmic}
% \label{alg1}
% \end{algorithm}
